Asymptotic normality of a linear threshold estimator in fixed dimension with near-optimal rate

Linear thresholding models postulate that the conditional distribution of a response variable in terms of covariates differs on the two sides of a (typically unknown) hyperplane in the covariate space. A key goal in such models is to learn about this separating hyperplane. Exact likelihood or least squares methods to estimate the thresholding parameter involve an indicator function which make them difficult to optimize and are, therefore, often tackled by using a surrogate loss that uses a smooth approximation to the indicator. In this paper, we demonstrate that the resulting estimator is asymptotically normal with a near optimal rate of convergence: $n^{-1}$ up to a log factor, in both classification and regression thresholding models. This is substantially faster than the currently established convergence rates of smoothed estimators for similar models in the statistics and econometrics literatures. We also present a real-data application of our approach to an environmental data set where $CO_2$ emission is explained in terms of a separating hyperplane defined through per-capita GDP and urban agglomeration.

==> Upload materials/Real_data_analysis.tex <==
% !TEX root = Final_draft.tex
\section{Real data analysis}
\label{sec:real_data}
We illustrate our method using cross-country data on pollution (carbon-dioxide), income and urbanization obtained from the World Development Indicators (WDI), World Bank. The Environmental Kuznets Curve hypothesis (EKC henceforth), a popular and ongoing area of research in environmental economics, posits that at an initial stage of economic development pollution increases with economic growth, and then diminishes when society’s priorities change, leading to an inverted U-shaped relation between income (measured via real GDP per capita) and pollution. The hypothesis has led to numerous empirical papers (i) testing the hypothesis (whether the relation is inverted U-shaped for countries/regions of interest in the sample), (ii) exploring the threshold level of income at which pollution starts falling, as well as (iii) examining the countries/regions which belong to the upward rising part versus the downward sloping part of the inverted U-shape, if at all. The studies have been performed using US state level data or cross-country data (e.g. \cite{shafik1992economic}, \cite{millimet2003environmental}, \cite{aldy2005environmental}, \cite{lee2019nonparametric},\cite{boubellouta2021cross}, \cite{list1999environmental}, \cite{grossman1995economic}, \cite{bertinelli2005environmental}, \cite{azomahou2006economic}, \cite{taskin2000searching} to name a few). While some of these papers have found evidence in favor of the EKC hypothesis (inverted U-shaped income-pollution relation), others have found evidence against it (monotonically increasing or other shapes for the relation). The results often depend on countries/regions in the sample, period of analysis, as well as the pollutant studied.
\\\\
\noindent
While income-pollution remains the focal point of most EKC studies, several of them have also included urban agglomeration (UA) or some other measures of urbanization as an important control variable especially while investigating carbon emissions.\footnote {Although income growth is connected to urbanization, countries are heterogenous and follow different growth paths due to their varying geographical structures, population densities, infrastructures, ownerships of resources making a case for using urbanization as another control covariate in the income-pollution study. The income growth paths of oil rich UAE, manufacturing based China, serviced based Singapore, low population density Canada (with vast land) are all different.} (see for example, \cite{shafik1992economic}, \cite{boubellouta2021cross}and \cite{liang2019urbanization}). The theory of ecological economics posits potentially varying effects of increased urbanization on pollution– (i) urbanization leading to more pollution (due to its close links with sanitations, dense transportations, and proximities to polluting manufacturing industries), (ii) urbanization potentially leading to less pollution based on ‘compact city theory’ (see \cite{burton2000compact}, \cite{capello2000beyond}, \cite{sadorsky2014effect}) that explains the potential benefits of increased urbanization in terms of economies of scale (for example, replacing dependence on automobiles with large scale subway systems, using multi-storied buildings instead of single unit houses, keeping more open green space). \cite{liddle2010age}, using 17 developed countries, find a positive and significant effect of urbanization on pollution. On the contrary, using a set of 69 countries \cite{sharma2011determinants} find a negative and significant effect of urbanization on pollution while \cite{du2012economic} find an insignificant effect of urbanization on carbon emission. Using various empirical strategies \cite{sadorsky2014effect} conclude that the positive and negative effects of urbanization on carbon pollution may cancel out depending on the countries involved often leaving insignificant effects on pollution. They also note that many countries are yet to achieve a sizeable level of urbanization which presumably explains why many empirical works using less developed countries find insignificant effect of urbanization.  In summary, based on the existing literature, both the relationship between urbanization and pollution as well as the relationship between income and pollution appear to depend largely on the set of countries considered in the sample. This motivates us to use UA along with income in our change plane model for analyzing carbon-dioxide emission to plausibly separate the countries into two regimes. 
\\\\
\noindent
Following the broad literature we use pollution emission per capita (carbon-dioxide measured in metric tons per capita) as the dependent variable and real GDP per capita (measured in 2010 US dollars), its square (as is done commonly in the EKC literature) and a popular measure of urbanization, namely urban agglomeration  (UA)\footnote{The exact definition can be found in the World Development Indicators database from the World Bank website.} as covariates (in our notation $X$) in our regression. In light of the preceding discussions we fit a change plane model comprising real GDP per capita and UA (in our notation $Q$). To summarize the setup, we use the continuous response model as described in equation \eqref{eq:regression_main_eqn}, i.e 
\begin{align*}
Y_i & = X_i^{\top}\beta_0 + X_i^{\top}\delta_0\mathds{1}_{Q_i^{\top}\psi_0 > 0} + \eps_i \\
& = X_i^{\top}\beta_0\mathds{1}_{Q_i^{\top}\psi_0 \le 0} + X_i^{\top}(\beta_0 + \delta_0)\mathds{1}_{Q_i^{\top}\psi_0 > 0} + \eps_i
\end{align*}
with the per capita $CO_2$ emission in metric ton as $Y$, per capita GDP, square of per capita GDP and UA as $X$ (hence $X \in \bbR^3$) and finally, per capita GDP and UA as $Q$ (hence $Q \in \bbR^2$). Observe that $\beta_0$ represents the regression coefficients corresponding to the countries with $Q_i^{\top}\psi_0 \le 0$ (henceforth denoted by Group 1) and $(\beta_0+ \delta_0)$ represents the regression coefficients corresponding to the countries with $Q_i^{\top}\psi_0 \ge 0$ (henceforth denoted by Group 2). As per our convention, in the interests of identifiability we assume $\psi_{0, 1} = 1$, where $\psi_{0,1}$ is the change plane parameter corresponding to per capita GDP. Therefore the only change plane coefficient to be estimated is $\psi_{0, 2}$, the change plane coefficient for UA. For numerical stability, we divide per capita GDP by $10^{-4}$ (consequently square of per capital GDP is scaled by $10^{-8}$)\footnote{This scaling helps in the numerical stability of the gradient descent algorithm used to optimize the least squares criterion.}.  After some pre-processing (i.e. removing rows consisting of NA and countries with $100\%$ UA) we estimate the coefficients $(\beta_0, \delta_0, \psi_0)$ of our model based on data from 115 countries with $\sigma_n = 0.05$ and test the significance of the various coefficients using the methodologies described in Section \ref{sec:inference}. We present our findings in Table \ref{tab:ekc_coeff}.  
\begin{table}[!h]
    \centering
    \begin{tabular}{|c||c||c|}
    \hline
    Coefficients & Estimated values & p-values \\
    \hline \hline 
      $\beta_{0, 1}$ (\text{RGDPPC for Group 1})  & 6.98555060 & 4.961452e-10   \\
       $\beta_{0, 2}$ (\text{squared RGDPPC for Group 1})  &  -0.43425991 & 7.136484e-02 \\
       $\beta_{0, 3}$ (\text{UA for Group 1}) & -0.02613813  & 1.066065e-01
\\
       $\beta_{0, 1} + \delta_{0, 1}$ (\text{RGDPPC for Group 2}) & 2.0563337 & 0.000000e+00\\
      $\beta_{0, 2} + \delta_{0, 2}$ (\text{squared RGDPPC for Group 2}) &  -0.1866490 & 4.912843e-04   \\
       $\beta_{0, 3} + \delta_{0, 3}$ (\text{UA for Group 2}) & 0.1403171& 1.329788e-05 \\
       $\psi_{0,2 }$  (\text{Change plane coeff for UA}) & -0.07061785 & 0.000000e+00\\
         \hline
    \end{tabular}
    \caption{Table of the estimated regression and change plane coefficients along with their p-values.}
    \label{tab:ekc_coeff}
\end{table}
\\\\
\noindent
From the above analysis, we find that GDP has significantly positive effect on pollution for both groups of countries. The effect of its squared term is negative for both groups; but the effect is significant for Group-2 consisting of mostly high income countries whereas its effect is insignificant (at the 5\% level) for the Group-1 countries (consisting of mostly low or middle income and few high income countries). Thus, not surprisingly, we find evidence in favor of EKC for the developed countries, but not for the mixed group.  Notably, Group-1 consists of a mixed set of countries like Angola, Sudan, Senegal, India, China, Israel, UAE etc., whereas Group-1 consists of rich and developed countries like Canada, USA, UK, France, Germany etc. The urban variable, on the other hand, is seen to have insignificant effect on Group-1 which is in keeping with \cite{du2012economic}, \cite{sadorsky2014effect}. Many of them are yet to achieve substantial urbanization and this is more true for our sample period \footnote{We use 6 years average from 2010-2015 for GDP and pollution measures. Such averaging is in accordance with the cross-sectional empirical literature using cross-country/regional data and helps avoid business cycle fluctuations in GDP. It also minimizes the impacts of outlier events such as the financial crisis or great recession period.  The years that we have chosen are ones for which we could find data for the largest number of countries.}. In contrast, UA has a positive and significant effect on Group-2 (developed) countries which is consistent with the findings of \cite{liddle2010age}, for example. Note that UA plays a crucial role in dividing the countries into different regimes, as the estimated value of $\psi_{0,2}$ is significant. Thus, we are able to partition countries into two regimes: a mostly rich and a mixed group. 
\\\\
\noindent
Note that many underdeveloped countries and poorer regions of emerging countries are still swamped with greenhouse gas emissions from burning coal, cow dung etc., and usage of poor exhaust systems in houses and for transport. This is more true for rural and semi-urban areas of developing countries. So even while being less urbanized compared to developed nations, their overall pollution load is high (due to inefficient energy usage and higher dependence on fossil fuels as pointed out above) and rising with income and they are yet to reach the descending part of the inverted U-shape for the income-pollution relation. On the contrary, for countries in Group-2, the adoption of more efficient energy and exhaust systems are common in households and transportations in general, leading to eventually decreasing pollution with increasing income (supporting EKC). Both the results are in line with the existing EKC literature. Additionally we find that the countries in Group 2 are yet to achieve ‘compact city’ and green urbanization. This is a stylized fact that is confirmed by the positive and significant effect of UA on pollution in our analysis.  
\\\\
\noindent
There are many future potential applications of our method in economics. Similar analyses can be performed for other pollutants (such as sulfur emission, electrical waste/e-waste, nitrogen pollution etc.). While income/GDP remains a common, indeed the most crucial variable in pollution studies, other covariates (including change plane defining variables) may vary, depending on the pollutant of interest. Another potential application can be that of identifying the determinants of family health expenses in household survey data. Families are often asked about their health expenses incurred in the past one year. An interesting case in point may be household surveys collected in India where one finds numerous (large) joint families with several children and old people residing in the same household and most families are uninsured. It is often seen that health expenditure increases with income with a major factor being the costs associated with regularly performed preventative medical examinations which are affordable only once a certain income level is reached. The important covariates here are per capita family income, family wealth, `dependency ratio' (number of children and old to the total number of people in the family) and the binary indicator of any history of major illness/hospitalizations in the family in the past year. Family income per capita and history of major illness are natural candidate covariates for defining the change plane. 


==> Upload materials/classification.tex <==
% !TEX root = main.tex
\section{Binary response model}
\label{sec:classification_analysis}
Recall our binary response model in equation \eqref{eq:classification_eqn}. To estimate $\psi_0$, we resort to the following  loss (without smoothing): 
\begin{equation}
\label{eq:new_loss}
\bbM(\psi) = \bbE\left((Y - \gamma)\mathds{1}(Q^{\top}\psi \le 0)\right)\end{equation}
with $\gamma \in (\alpha_0, \beta_0)$, which can be viewed as a variant of the square error loss function: 
$$
\bbM(\alpha, \beta, \psi) = \bbE\left(\left(Y - \alpha\mathds{1}(Q^{\top}\psi < 0) - \beta\mathds{1}(Q^{\top}\psi > 0)\right)^2\right)\,.
$$
We establish the connection between these losses in sub-section \ref{loss_func_eq}. It is easy to prove that under fairly mild conditions (discussed later) 
$\psi_0 = \argmin_{\psi \in \Theta}\bbM(\psi)$, uniquely. Under the standard classification paradigm, when we know a priori that 
$\alpha_0 < 1/2 < \beta_0$, we can take $\gamma = 1/2$, and in the absence of this constraint, $\bar{Y}$, which converges to some $\gamma$ between $\alpha_0$ and $\beta_0$, may be substituted in the loss function. In the rest of the paper, we confine ourselves to a known $\gamma$, and for technical simplicity, we take $\gamma = \frac{(\beta_0 + \alpha_0)}{2}$, but this assumption can be removed with more mathematical book-keeping. Thus, $\psi_0$ is estimated by:  
\begin{equation}
\label{non-smooth-score} 
\hat \psi = \argmin_{\psi \in \Theta} \mathbb{M}_n(\psi) = \argmin_{\psi \in \Theta} \frac{1}{n}\sum_{\i=1}^n (Y_i - \gamma)\mathds{1}(Q_i^{\top}\psi \le 0)\,.
\end{equation} We resort to a smooth approximation of the indicator function in 
\eqref{non-smooth-score} using a distribution kernel with suitable bandwidth. The smoothed version of the population score function then becomes: 
\begin{equation}
\label{eq:kernel_smoothed_pop_score}
\bbM^s(\psi) = \bbE\left((Y - \gamma)\left(1-K\left(\frac{Q^{\top}\psi}{\sigma_n}\right)\right)\right)
\end{equation}
where as in the continuous response model, we use $K(x) = \Phi(x)$, and the corresponding empirical version is: 
\begin{equation}
\label{eq:kernel_smoothed_emp_score}
\bbM^s_n(\psi) = \frac{1}{n}\sum_{i=1}^n \left((Y_i - \gamma)\left(1-K\left(\frac{Q_i^{\top}\psi}{\sigma_n}\right)\right)\right)
\end{equation}
Define $\hat{\psi}^s$ and $\psi_0^s$ to be the minimizer of the smoothed version of the empirical (equation \eqref{eq:kernel_smoothed_emp_score}) and population score (equation \eqref{eq:kernel_smoothed_pop_score}) function respectively. Here we only consider the choice of bandwidth $n\sigma_n \to \infty$ and $n\sigma_n^2 \to 0$. Analogous to Theorem \ref{thm:regression} we prove the following result for binary response model: 
\begin{theorem}
\label{thm:binary}
Under Assumptions (\ref{as:distribution} - \ref{as:eigenval_bound}): 
$$
\sqrt{\frac{n}{\sigma_n}}\left(\hat{\psi}_n - \psi_0\right) \Rightarrow N(0, \Gamma) \,,
$$ 
for some non-stochastic matrix $\Gamma$, which will be defined explicitly in the proof. 
\end{theorem}
We have therefore established that in the regime $n\sigma_n \to \infty$ and $n\sigma_n^2 \to 0$, it is possible to attain asymptotic normality using a smoothed estimator for binary response model. 





\section{Inferential methods}
\label{sec:inference}
We draw inferences on $(\beta_0, \delta_0, \psi_0)$ by resorting to similar techniques as in \cite{seo2007smoothed}. For the continuous response model, we need consistent estimators of $V^{\gamma}, Q^{\gamma}, V^{\psi}, Q^{\psi}$ (see Lemma \ref{conv-prob} for the definitions) for hypothesis testing. By virtue of the aforementioned Lemma, we can estimate $Q^{\gamma}$ and $Q^{\psi}$ as follows: 
\begin{align*}
\hat Q^{\gamma} & = \nabla^2_{\gamma} \bbM_n^s(\hat \theta) \,, \\ 
\hat Q^{\psi} & = \sigma_n \nabla^2_{\psi} \bbM_n^s(\hat \theta) \,.
\end{align*}
The consistency of the above estimators is established in the proof of Lemma \ref{conv-prob}. For the other two parameters $V^{\gamma}, V^{\psi}$ we use the following estimators: 
\begin{align*}
\hat V^{\psi} & = \frac{1}{n\sigma_n^2}\sum_{i=1}^n\left(\left(Y_i - X_i^{\top}(\hat \beta + \hat \delta)\right)^2 - \left(Y_i- X_i^{\top}\hat \beta\right)^2\right)^2\tilde Q_i \tilde Q_i^{\top}\left(K'\left(\frac{Q_i^{\top}\hat \psi}{\sigma_n}\right)\right)^2 \\
\hat V^{\gamma} & = \hat \sigma^2_\eps \begin{pmatrix} \frac{1}{n}X_iX_i^{\top} & \frac{1}{n}X_iX_i^{\top}\mathds{1}_{Q_i^{\top}\hat \psi > 0} \\ \frac{1}{n}X_iX_i^{\top}\mathds{1}_{Q_i^{\top}\hat \psi > 0} & \frac{1}{n}X_iX_i^{\top}\mathds{1}_{Q_i^{\top}\hat \psi > 0} \end{pmatrix}
\end{align*}
where $\hat \sigma^2_\eps$ can be obtained as $(1/n)(Y_i - X_i^{\top}\hat \beta - X_i^{\top}\hat \delta \mathds{1}(Q_i^{\top}\hat \psi > 0))^2$, i.e. the residual sum of squares. The explicit value of $V_\gamma$ (as derived in equation \eqref{eq:def_v_gamma} in the proof Lemma \ref{asymp-normality}) is: 
$$
V^{\gamma} = \sigma_\eps^2 \begin{pmatrix}\bbE\left[XX^{\top}\right] & \bbE\left[XX^{\top}\mathds{1}_{Q^{\top}\psi_0 > 0}\right] \\
\bbE\left[XX^{\top}\mathds{1}_{Q^{\top}\psi_0 > 0}\right] & \bbE\left[XX^{\top}\mathds{1}_{Q^{\top}\psi_0 > 0}\right] \end{pmatrix} 
$$ 
Therefore, the consistency of $\hat V_\gamma$ is immediate from the law of large numbers. The consistency of $\hat V^{\psi}$ follows via arguments similar to those employed in proving Lemma \ref{conv-prob} but under somewhat more stringent moment conditions: in particular, we need $\bbE[\|X\|^8] < \infty$ and $\bbE[(X^{\top}\delta_0)^k \mid Q]$ to be Lipschitz functions over $Q$ for $1 \le k \le 8$. The inferential techniques for the classification model are similar and hence skipped, to avoid repetition. 





%\subsection{Proof sketch }
%\label{sec:proof}
%The proof of the theorem is relatively long, so we break it into several lemmas. We  provide a roadmap of the proof in this section while the elaborate technical derivations of the supporting lemmas are relegated to section 4. 
%Define the following: $$T_n(\theta) = \nabla \mathbb{M}_n(\theta) = -\frac{1}{n\sigma_n}\sum_{i=1}^n (Y_i - \gamma)k\left(\frac{X_i^{\top}\theta}{\sigma_n}\right)\tilde{Q}_i$$ $$Q_n(\theta) = \nabla^2 \mathbb{M}_n(\theta) = -\frac{1}{n\sigma_n^2}\sum_{i=1}^n (Y_i - \gamma)k'\left(\frac{X_i^{\top}\theta}{\sigma_n}\right)\tilde{Q}_i\tilde{Q}_i^{\top}$$ As $\hat{\theta}_n$ minimizes $\mathbb{M}_n(\theta)$ we have $T_n(\hat{\theta}_n) = 0$. Using one step Taylor expansion we have:
%\allowdisplaybreaks 
%\begin{align*}
%T_n(\hat{\theta}_n) = T_n(\theta_0) + Q_n(\bar{\theta}_n)\left(\hat{\theta}_n - \theta_0\right) = 0
%\end{align*}
%or: 
%\begin{equation}
%\label{eq:main_eq}  \sqrt{n/\sigma_n}\left(\hat{\theta}_n - \theta_0\right) = -\left(\sigma_nQ_n(\bar{\theta}_n)\right)^{-1}\sqrt{n\sigma_n}T_n(\theta_0) 
%\end{equation}
%for some intermediate point $\bar{\theta}_n$ between $\hat \theta_n$ and $\theta_0$. The following lemma establishes the asymptotic properties of $T_n(\theta_0)$: 
%\begin{lemma}[Asymptotic Normality of $T_n$]
%\label{asymp-normality}
%%\begin{lemma}
%\label{asymp-normality}
%For a kernel $K$ satisfying the conditions of Assumption \ref{as:kernel} and with $n\sigma_n^{3} \rightarrow \lambda$, then $$\sqrt{n \sigma_n} T_n(\theta_0) \Rightarrow \mathcal{N}(\mu, \Sigma)$$ where $$\mu = -\sqrt{\lambda}\frac{\beta_0 - \alpha_0}{2}\left[\int_{-1}^{1} k\left(t\right)|t| \ dt \right] \int_{\mathbb{R}^{p-1}}\tilde{Q} f'(0 | \tilde{Q}) \ dP(\tilde{Q})$$ and $$\Sigma = \left[a_1 \int_{-1}^{0} \left(k\left(t\right)\right)^2  \ dt + a_2 \int_{0}^{1} \left(k\left(t\right)\right)^2 \ dt \right]\int_{\mathbb{R}^{p-1}}\tilde{Q}\tilde{Q}^{\top} f(0|\tilde{Q})  \ dP(\tilde{Q}) \,.$$ 
%Here $a_1 = (1 - \gamma)^2 \alpha_0 + \gamma^2 (1-\alpha_0), a_2 = (1 - \gamma)^2 \beta_0 + \gamma^2 (1-\beta_0)$ and $\alpha_0, \beta_0, \gamma$ are model parameters defined around equation \eqref{eq:new_loss}. 
%\end{lemma}
%\noindent
%%If we take $\sigma_n$ to be close to $1/n$ say $\sigma_n = (\log{n})^2/n$ then $\lambda = 0$. 
%In the case that $n \sigma_n^3 \rightarrow 0$, which, holds when $\log n/(n\sigma_n) \rightarrow 0$ as assumed prior to the statement of the theorem, $\lambda = 0$ and we have: 
%$$\sqrt{n \sigma_n} T_n(\theta_0) \rightarrow \mathcal{N}(0, \Sigma) \,.$$ 
%Next, we analyze the convergence of $Q_n(\bar{\theta}_n)^{-1}$ which is stated in the following lemma: 
%\begin{lemma}[Convergence in Probability of $Q_n$]
%\label{conv-prob}
%Under Assumptions (\ref{as:distribution} - \ref{as:eigenval_bound}), for any random sequence $\breve{\theta}_n$ such that $\|\breve{\theta}_n - \theta_0\|/\sigma_n \overset{P} \rightarrow 0$, $$\sigma_n Q_n(\breve{\theta}_n) \overset{P} \rightarrow Q = \frac{\beta_0 - \alpha_0}{2}\left(\int_{-1}^{1} -k'\left(t \right)\s(t) \ dt\right) \ \bbE\left(\tilde{Q}\tilde{Q}^{\top} f(0 |\tilde{Q})\right) \, .$$
%\end{lemma}
%It will be shown later that the condition $\|\breve{\theta}_n - \theta_0\|/\sigma_n \overset{P} \rightarrow 0$ needed in Lemma \ref{conv-prob} holds for the (random) sequence $\bar \theta_n$. Then, combining Lemma \ref{asymp-normality} and Lemma \ref{conv-prob} we conclude from equation \ref{eq:main_eq} that: $$\sqrt{n/\sigma_n} \left(\hat{\theta}_n - \theta_0\right) \Rightarrow N(0, Q^{-1}\Sigma Q^{-1})$$ This concludes the proof of the our Theorem \ref{main} with $\Gamma = Q^{-1}\Sigma Q^{-1}$. 
%\newline
%\newline
%Observe that, to show $\left\|\bar \theta_n - \theta_0 \right\| = o_P(\sigma_n)$, it suffices to to prove that $\left\|\hat \theta_n - \theta_0 \right\| = o_P(\sigma_n)$. Towards that direction, we have following lemma: 
%
%\begin{lemma}[Rate of convergence]
%\label{lem:rate}
%Under Assumptions (\ref{as:distribution} - \ref{as:eigenval_bound}), 
%$$n^{2/3}\sigma_n^{-1/3} d^2_n\left(\hat \theta_n, \theta_n\right) = O_P(1)$$ where $$d_n\left(\theta, \theta_n\right) = \sqrt{\left[\frac{\|\theta - \theta_n\|^2}{\sigma_n} \mathds{1}(\|\theta - \theta_n\| \le \cK\sigma_n) + \|\theta - \theta_n\|  \mathds{1}(\|\theta - \theta_n\| \ge \cK\sigma_n)\right]}$$ for some specific constant $\cK$. (This constant will be mentioned precisely in the proof). Hence as $n\sigma_n \to \infty$, we have $n^{2/3}\sigma_n^{-1/3} \gg \sigma_n^{-1}$ which implies $\frac{\|\hat{\theta}_n - \theta_n\|}{\sigma_n}  \overset{P}  \longrightarrow 0 \,.$
%\end{lemma}
%
%\noindent
%The lemma immediately leads to the following corollary: 
%
%\begin{corollary}
%\label{rate-cor}
%If $(\log{n})/(n\sigma_n)\rightarrow 0$ then $\frac{\|\hat{\theta}_n - \theta_n\|}{\sigma_n}  \overset{P}  \longrightarrow 0$
%\end{corollary}
%
%\noindent
%Finally, to establish $\|\hat{\theta}_n - \theta_0\|/\sigma_n \overset{P} \rightarrow 0$, all we need is that $\|\theta_n - \theta_0\|/\sigma_n \rightarrow 0$ as demonstrated in the following lemma:
%
%\begin{lemma}[Convergence of population minimizer]
%\label{bandwidth}
%If the smoothing kernel satisfies Assumption \ref{as:kernel}, then for any sequence of $\sigma_n \rightarrow 0$, we have: $\|\theta_n - \theta_0\|/\sigma_n \rightarrow 0$. 
%\end{lemma}
%
%\noindent
%Hence the final roadmap is the following: Using Lemma \ref{bandwidth} and Corollary \ref{rate-cor} we establish that $\|\hat{\theta}_n - \theta_0\|/\sigma_n \rightarrow 0$ if $\log{n}/(n\sigma_n) \rightarrow 0$. This, in turn, enables us to prove that $\sigma_n Q_n(\bar{\theta}_n) \overset{P} \rightarrow Q$,which, along with Lemma \ref{asymp-normality}, establishes the main theorem. 
%\\\\
%\begin{remark}
%\label{sub-gaussian-assumption} 
%One may wonder whether the subgaussian assumption on the distribution of $X$ can be relaxed. We use this condition to prove Lemma \ref{conv-prob}. The fact that $\breve{\theta}$ defined in this Lemma is a random sequence necessitates the use of a Glivenko-Cantelli type result. This is facilitated by the subgaussianity assumption on the distribution of $X$ which allows us to apply a certain maximal inequality. It may be possible to relax the assumption if one is willing to use more sophisticated inequalities, but we have not explored this direction. 
%\end{remark} 



==> Upload materials/joe_main.tex <==
% !TEX root = main.tex
\section{Introduction}
The simple linear regression model assumes a uniform linear relationship between the covariate and the response, in the sense that the regression parameter $\beta$ is the same over the entire covariate domain. In practice, the situation can be more complicated: for instance, the regression parameter may differ from sub-population to sub-population within a large (super-) population. Some common techniques to account for such heterogeneity include mixed linear models, introducing an interaction effect, or fitting different models among each sub-population which corresponds to a supervised classification setting where the true groups (sub-populations) are \emph{a priori known}. 
	\newline
	\newline
	\indent A more difficult scenario arises when the sub-populations are unknown, in which case regression and classification must happen simultaneously. Consider the scenario where the conditional mean of $Y_i$ given $X_i$ is different for different unknown sub-groups. A  well-studied treatment of this problem -- the so-called change point problem -- considers a simple thresholding model where membership in a sub-group is determined by whether a real-valued observable $X$ falls to the left or right of an unknown parameter $\gamma$. More recently, there has been work for multi-dimensional covariates, namely when the membership is determined by which side a random vector $X$ falls with respect to an hyperplane with unknown normal vector $\theta_0$. A concrete example appears in \cite{wei2014latent} who extend the linear thresholding model due to  \cite{kang2011new} to general dimensions: 
	\begin{eqnarray}\label{eq:weimodel}
	Y=\mu_1\cdot 1_{X^{\top}\theta_0\geq 0}+\mu_2\cdot 1_{X^{\top}\theta_0<0}+\varepsilon\,,
	\end{eqnarray}
	and studied computational algorithms and consistency of the same. This model and others with similar structure, called \emph{change plane models}, are useful in various fields of research, e.g. modeling treatment effect heterogeneity in drug treatment (\cite{imai2013estimating}), modeling sociological data on voting and employment (\cite{imai2013estimating}), or cross country growth regressions in econometrics 
(\cite{seo2007smoothed}).
	\newline
	\newline
\indent Other aspects of this model have also been investigated. \cite{fan2017change} examined the change plane model from the statistical testing point of view, with the null hypothesis being the absence of a separating hyperplane. They proposed a test statistic, studied its asymptotic distribution and provided sample size recommendations for achieving target values of power. \cite{li2018multi} extended the change point detection problem in the multi-dimensional setup by considering the case where $X^{\top}\theta_0$ forms a multiple change point data sequence. 
	%In parallel with this, \cite{bai1998estimating} considered estimation of a multiple change point model with an iterative method, where at each step, a statistical test was performed on the existence of an additional change point. 
The key difficultly with change plane type models is the inherent discontinuity in the optimization criteria involved where the parameter of interest appears as an argument to some indicator function, rendering the optimization extremely hard. To alleviate this, one option is to kernel smooth the indicator function, an approach that was adopted by Seo and Linton \cite{seo2007smoothed} in a version of the change-plane problem, motivated by earlier results of Horowitz \cite{horowitz1992smoothed} that dealt with a smoothed version of the maximum score estimator. Their model has an additive structure of the form:
\[Y_t = \beta^{\top}X_t + \delta^{\top} \tilde{X}_t \mathds{1}_{Q_t^{\top} \boldmath \psi > 0} + \epsilon_t \,,\]
where $\psi$ is the (fixed) change-plane parameter, and $t$ can be viewed as a time index. Under a set of assumptions on the model (Assumptions 1 and 2 of their paper), they showed asymptotic normality of their estimator of $\psi$ obtained by minimizing a smoothed least squares criterion
that uses a differentiable distribution function $\mathcal{K}$. The rate of convergence of $\hat{\psi}$ to the truth was shown to be $\sqrt{n/\sigma_n}$ where $\sigma_n$ was the bandwidth parameter used to smooth the least squares function. As noted in their Remark 3, under the special case of i.i.d. observations, their requirement that $\log n/(n \sigma_n^2) \rightarrow 0$ translates to a maximal convergence rate of $n^{3/4}$ up to a logarithmic factor. The work of \cite{li2018multi} who considered multiple parallel change planes (determined by a fixed dimensional normal vector) and high dimensional linear models in the regions between consecutive hyperplanes also builds partly upon the methods of \cite{seo2007smoothed} and obtains the same (almost) $n^{3/4}$ rate for the normal vector (as can be seen by putting Condition 6 in their paper in conjunction with the conclusion of Theorem 3). 
\\\\

While it is established that the condition $n\sigma_n^2 \to \infty$ is sufficient (upto a log factor) for achieving asymptotic normality of the smoothed estimator, there is no result in the existing literature to ascertain whether its necessity. Intuitively speaking, the necessary condition for asymptotic normality ought to be $n \sigma_n \to 0$, as this will ensure a growing number of observations in a $\sigma_n$ neighborhood around the true hyperplane, allowing the central limit theorem to kick in. In this paper we \emph{bridge this gap} by proving that asymptotic normality of the smoothed change point estimator is, in fact, achievable with $n \sigma_n \to \infty$. 
%\footnote{In fact, we strongly believe that the additional conditional $n^{1/4}\sigma_n \to 0$ is necessary for the effect of the bias introduced by smoothing the indicator function to be asymptotically negligible. Details can be found in the proof of Theorem \ref{}.}. 
This implies that the best possible rate of convergence of the smoothed estimator can be arbitrarily close to $n^{-1}$, the minimax optimal rate of estimation for this problem. To demonstrate this, we focus on two change plane estimation problems, one with a continuous and another with a binary response. The continuous response model we analyze here is the following: 
\begin{equation}
\label{eq:regression_main_eqn}
Y_i = \beta_0^{\top}X_i + \delta_0^{\top}X_i\mathds{1}_{Q_i^{\top}\psi_0 > 0} + \eps_i \,.
\end{equation}
for i.i.d. observations $\{(X_i, Y_i, Q_i\}_{i=1}^n$, where the zero-mean transitory shocks $\eps_i \indep (X_i, Q_i)$. Our calculation can be easily extended to the case when the covariates on the either side of the change hyperplane are different and $\bbE[\eps \mid X, Q] = 0$ with more tedious bookkeeping. As this generalization adds little of interest, conceptually, to our proof, we posit the simpler model for ease of understanding.
%In comparison to the model analyzed in \cite{seo2007smoothed}, we use the following three simplifications: (1) we assume $\tilde X = X$. (2) $\eps \indep (X, Q)$ and (3) the observations are i.i.d. The first and second simplifications are for mathematical convenience: our proof can be easily extended to the case when $\tilde X \neq X$ and $E(\eps \mid X, Q) = 0$.  To relax the third condition to the case of non i.i.d. samples (e.g. introducing some short range dependence as in \citep{seo2007smoothed}) will need some refinement of the current techniques to accommodate the dependence structure. As the calculation for i.i.d. data is already highly involved and cumbersome and the i.i.d. setting covers many interesting cross-sectional applications (one of which is presented in Section \ref{sec:real_data}), we confine ourselves to the independent observations case.  
As the parameter $\psi_0$ is only identifiable upto its norm, we assume that the first co-ordinate is $1$ (along the lines of \cite{seo2007smoothed}) which removes one degree of freedom and makes the parameter identifiable. 
\\\\
To illustrate that a similar phenomenon transpires with binary response, we also study a canonical version of such a model which can be briefly described as follows: The covariate $Q \sim P$ where $P$ is distribution on $\mathbb{R}^d$ and the conditional distribution of $Y$ given $Q$ is modeled as follows: 
\begin{equation}
\label{eq:classification_eqn}
P(Y=1|Q) = \alpha_0 \mathds{1}(Q^{\top}\psi_0 \le 0) + \beta_0\mathds{1}(Q^{\top}\psi_0 > 0)
\end{equation}
for some parameters $\alpha_0, \beta_0\in (0,1)$ and $\psi_0\in\mathbb{R}^d$ (with first co-ordinate being one for identifiability issue as for the continuous response model), the latter being of primary interest for estimation. 
This model is identifiable up to a permutation of $(\alpha_0, \beta_0)$, so we further assume $\alpha_0 < \beta_0$. For both models, we show that $\sqrt{n/\sigma_n}(\hat \psi - \psi_0)$ converges to zero-mean normal distribution as long as $n \sigma_n \to \infty$ but the calculations for the binary model are completely relegated to Appendix \ref{sec:supp_classification}. 
%Our goal is to show that a kernel-smoothed version of an appropriate loss function in this problem can produce estimates of $\theta_0$ that converge at a rate \emph{logarithmically close to $1/n$}, and are asymptotically normal under a set of reasonable assumptions on the underlying model. Our message here is that while smoothing the indicator function does compromise the rate of convergence relative to the exact least squares/maximum likelihood estimator, a fact also noted in \cite{seo2007smoothed}, the compromise can be quite minimal (i.e. to within a logarithmic factor of the best rate). We note that the rate obtained here is faster than the one obtained by \cite{seo2007smoothed} in their model, which while being different in certain aspects -- ours is a classification problem and theirs a regression, and the model assumptions are also not fully comparable, but both have the same fundamental structure of a jump discontinuity at a separating hyperplane. We expect that our convergence rate should arise in many different incarnations of the change-plane model under fairly reasonable assumptions. At a more technical level, we are able to obtain a faster convergence rate for the normal vector to the hyperplane in comparison to \cite{seo2007smoothed} and \cite{li2018multi} as our techniques allow us to impose a weaker restriction on our smoothing bandwidth $\sigma_n$: we only require $\log n /(n \sigma_n) \rightarrow 0$ in contrast to the (stronger) constraint $\log n/(n \sigma_n^2) \rightarrow 0$ in Seo and Linton's work. The details appear later in the paper. 
\\\\
{\bf Organization of the paper:} The rest of the paper is organized as follows: In Section \ref{sec:theory_regression} we present the methodology, the statement of the asymptotic distributions and a sketch of the proof for the continuous response model \eqref{eq:regression_main_eqn}. In Section \ref{sec:classification_analysis} we briefly describe the binary response model \eqref{eq:classification_eqn} and related assumptions, whilst the details can be found in the supplementary document. In Section \ref{sec:simulation} we present some simulation results, both for the binary and the continuous response models to study the effect of the bandwidth on the quality of the normal approximation in finite samples. In Section \ref{sec:real_data}, we present a real data analysis where we analyze the effect of  income and urbanization on the $CO_2$ emission in different countries. 
\\\\
{\bf Notations: } Before delving into the technical details, we first setup some notations here. We assume from now on, $X \in \reals^p$ and $Q \in \reals^d$. For any vector $v$ we define by $\tilde v$ as the vector with all the co-ordinates expect the first one. We denote by $K$ the kernel function used to smooth the indicator function. For any matrix $A$, we denote by $\|A\|_2$ (or $\|A\|_F$) as its Frobenious norm and $\|A\|_{op}$ as its operator norm. For any vector, $\| \cdot \|_2$ denotes its $\ell_2$ norm.  






%
%
%
%
%To estimate $\theta_0$ in the discrete version of the model, we resort to the following  loss: 
%\begin{equation}
%\label{eq:new_loss}
%M(\theta) = \bbE\left((Y - \gamma)\mathds{1}(X^{\top}\theta \le 0)\right)\end{equation}
%with $\gamma \in (\alpha_0, \beta_0)$, which can be viewed as a variant of the squared error loss function: 
%$$M^{(LS)}(\alpha, \beta, \theta) = \bbE\left(\left(Y - \alpha\mathds{1}(X^{\top}\theta < 0) - \beta\mathds{1}(X^{\top}\theta > 0)\right)^2\right)\,.$$
%We establish the connection between these losses in sub-section \ref{loss_func_eq}. It is easy to prove that under fairly mild conditions (discussed later) 
%$\theta_0 = \argmin_{\theta \in \Theta}M(\theta)$, uniquely. Under the standard classification paradigm, when we know a priori that 
%$\alpha_0 < 1/2 < \beta_0$, we can take $\gamma = 1/2$, and in the absence of this constraint, $\bar{Y}$, which converges to some $\gamma$ between $\alpha_0$ and $\beta_0$, may be substituted in the loss function. In the rest of the paper, we confine ourselves to a known $\gamma$, and for technical simplicity, we take $\gamma = \frac{(\beta_0 + \alpha_0)}{2}$, but this assumption can be removed quite easily at the cost of a non-zero mean in the limiting normal distribution derived in Theorem \ref{main}. Thus, $\theta_0$ is estimated by:  
%\begin{equation}
%\label{non-smooth-score} 
%\theta_n^{\dagger} = \argmin_{\theta \in \Theta} \mathbb{M}_n(\theta) = \argmin_{\theta \in \Theta} \frac{1}{n}\sum_{\i=1}^n (Y_i - \gamma)\mathds{1}(X_i^{\top}\theta \le 0)\,.
%\end{equation} We resort to a smooth approximation of the indicator function in 
%\eqref{non-smooth-score} using a distribution kernel with suitable bandwidth. The smoothed version of the population score function then becomes: 
%\begin{equation}
%\label{eq:kernel_smoothed_pop_score}
%M_n(\theta) = \bbE\left((Y - \gamma)\left(1-K\left(\frac{X^{\top}\theta}{\sigma_n}\right)\right)\right)
%\end{equation}
%where we take $K$ to be a twice-differentiable probability distribution function supported on $[-1,1]$ with symmetric density (see Assumption \ref{as:kernel}), and the corresponding empirical version is: 
%\begin{equation}
%\label{eq:kernel_smoothed_emp_score}
%\bbM_n(\theta) = \frac{1}{n}\sum_{i=1}^n \left((Y_i - \gamma)\left(1-K\left(\frac{X_i^{\top}\theta}{\sigma_n}\right)\right)\right)
%\end{equation}
%
%
%
%
%
%
%
%
%
%
%\section{Theoretical analysis}
\input{regression.tex}
\input{classification.tex}

\section{Simulation studies}
\label{sec:simulation}
In this section, we present some simulation results to analyse the effect of the choice of $\sigma_n$ on the finite sample approximation of asymptotic normality, i.e. Berry-Essen type bounds. If we choose a smaller sigma, the rate of convergence is accelerated but the normal approximation error at smaller sample sizes will be higher, as we don't have enough observations in the vicinity of the change hyperplane for the CLT to kick in. This problem is alleviated by choosing $\sigma_n$ larger, but this, on the other hand, compromises the convergence rate. Ideally, a Berry-Essen type of bound will quantify this, but this will require a different set of techniques and is left as an open problem. In our simulations, we generate data from following setup: 
\begin{enumerate}
\item Set $N = 50000, p = 3, \alpha_0 = 0.25, \beta = 0.75$ and some $\theta_0 \in \bbR^p$ with first co-ordinate $ = 1$. 
\item Generate $X_1, \dots, X_n \sim \cN(0, I_p)$. 
\item Generate $Y_i \sim \textbf{Bernoulli}\left(\alpha_0\mathds{1}_{X_i^{\top}\theta_0 \le 0} + \beta_0 \mathds{1}_{X_i^{\top}\theta_0 > 0}\right)$. 
\item Estimate $\hat \theta$ by minimizing $\bbM_n(\theta)$ (replacing $\gamma$ by $\bar Y$) based on $\{(X_i, Y_i)\}_{i=1}^n$ for different choices of $\sigma_n$. 
\end{enumerate}
We repeat Step 2 - Step 4 a hundred times to obtain $\hat \theta_1, \dots, \hat \theta_{100}$. Define $s_n$ to be the standard deviation of $\{\hat \theta_i\}_{i=1}^{100}$. Figures ref{fig:co2} and \ref{fig:co3} show the qqplots of $\tilde \theta_i = (\hat \theta_i - \theta_0)/s_n$ against the standard normal for four different choices of $\sigma_n = n^{-0.6}, n^{-0.7}, n^{-0.8}, n^{-0.9}$. 
\begin{figure}
\centering 
\includegraphics[scale=0.4]{Coordinate_2}
\caption{In this figure, we present qqplot for estimating second co-ordinate of $\theta_0$ with different choices of $\sigma_n$ mentioned at the top of each plots.}
\label{fig:co2}
\end{figure}
\begin{figure}
\centering 
\includegraphics[scale=0.4]{Coordinate_3}
\caption{In this figure, we present qqplot for estimating third co-ordinate of $\theta_0$ with different choices of $\sigma_n$ mentioned at the top of each plots.}
\label{fig:co3}
\end{figure}
It is evident that smaller value of $\sigma_n$ yield a poor normal approximation. Although our theory shows that asymptotic normality holds as long as $n\sigma_n \to \infty$, in practice we recommend choosing $\sigma_n$ such that $n\sigma_n \ge 30$ for the central limit of theorem to take effect. 



\begin{comment}
\section{Real data analysis}
\label{sec:real_data}
%In the real data analysis, our response variable is $Y$ is $CO_2$ emission per capita per metric ton, $X$ is the covariate sets containing GDP per capita (scaled by $10^4$), square of GDP per capita (scaled by $10^8$) and Urban agglomeration (henceforth UA). The change plane variables $Q$ contains GDP per capita (scaled by $10^4$) and UA. The following is the regression result of $Y$ on $X$ (without change plane):
%\begin{verbatim}
%Call:
%lm(formula = Y ~ X - 1)
%
%Residuals:
%    Min      1Q  Median      3Q     Max 
%-5.7076 -1.3180 -0.6318  0.3212 12.1995 
%
%Coefficients:
%                  Estimate Std. Error t value Pr(>|t|)    
%Xgdp_ave_vec       4.03525    0.49667   8.125 6.25e-13 ***
%X                 -0.42489    0.07473  -5.686 1.04e-07 ***
%XUrban_agglo_2015  0.04459    0.01593   2.799  0.00603 ** 
%---
%Signif. codes:  0 ‘***’ 0.001 ‘**’ 0.01 ‘*’ 0.05 ‘.’ 0.1 ‘ ’ 1
%
%Residual standard error: 3.06 on 113 degrees of freedom
%Multiple R-squared:  0.7818,	Adjusted R-squared:  0.776 
%F-statistic:   135 on 3 and 113 DF,  p-value: < 2.2e-16
%\end{verbatim}
%
%We next estimate the change plane problem using $\sigma_n = 0.05$. For initial point, we start with a grid search, find the point which minimizes the squared error loss and then do gradient descent using Normal cdf kernel. The final estimate is $\hat \psi^s = -0.05553278$. Using this change point estimate, our final estimate of regression coefficients $\hat \beta^s, \hat \delta^s$ is obtained by regressing $Y$ on $X$ and $X\mathds{1}_{Q^{\top}\hat \psi^s > 0}$: 
%
%
%
%\begin{verbatim}
%Call:
%lm(formula = Y ~ alternate_covs + primary_covs - 1)
%
%Residuals:
%    Min      1Q  Median      3Q     Max 
%-7.7724 -0.8396 -0.0581  1.0139  9.0144 
%
%Coefficients:
%                               Estimate Std. Error t value Pr(>|t|)    
%alternate_covsgdp_ave_vec       7.22097    1.07875   6.694 9.52e-10 ***
%alternate_covs                 -1.03085    0.20647  -4.993 2.25e-06 ***
%alternate_covsUrban_agglo_2015 -0.01954    0.02174  -0.899 0.370720    
%primary_covsgdp_ave_vec        -5.47001    1.22526  -4.464 1.95e-05 ***
%primary_covs                    0.85098    0.22050   3.859 0.000192 ***
%primary_covsUrban_agglo_2015    0.22358    0.03892   5.745 8.31e-08 ***
%---
%Signif. codes:  0 ‘***’ 0.001 ‘**’ 0.01 ‘*’ 0.05 ‘.’ 0.1 ‘ ’ 1
%
%Residual standard error: 2.683 on 110 degrees of freedom
%Multiple R-squared:  0.8367,	Adjusted R-squared:  0.8278 
%F-statistic: 93.96 on 6 and 110 DF,  p-value: < 2.2e-16
%\end{verbatim}
%
%We also have (from the gradient descent): 
%$$
%\hat \beta^s = \begin{pmatrix} 6.98231308 \\ -1.01996040 \\ -0.01503167 \end{pmatrix}, \hat \delta^s = \begin{pmatrix} -5.460687 \\ 0.859626 \\ 0.241815\end{pmatrix}
%$$
%which implies: 
%$$
%\hat \beta^s + \hat \delta^s = \begin{pmatrix}1.5216260 \\ -0.1603344 \\ 0.2267834 \end{pmatrix} \,.
%$$
%Further we test $\beta_{0, i} = 0$ for $1 \le i \le 3$ and $\beta_{0, i} + \delta_{0, i} = 0$ for $1 \le i \le 3$ based on our asymptotic result. We reject $H_0$ on all the coefficients except $\beta_{0, 3}$, which is the negative coefficient for UA corresponding to the countries for which $Q_i^{\top}\hat \psi^s \le 0$. The p-values corresponding these six tests are: $(4.817591e-11, 3.904592e-07, 2.446152e-01, 0.000000e+00, 0.000000e+00, 3.430589e-14)$. 
%\\\\
%\noindent
%Now we do regression on each group separately: note that the groups are closed to \emph{developed country} and \emph{developing countries/under-developed countries}. 
%\\\\
%\noindent
%{\bf Countries where $Q_i^{\top}\hat \psi^s \le 0$: }
%\begin{verbatim} 
%[1] "Afghanistan"        "Angola"             "Argentina"          "Armenia"           
% [5] "Azerbaijan"         "Bangladesh"         "Belarus"            "Bolivia"           
% [9] "Brazil"             "Bulgaria"           "Burkina Faso"       "Cambodia"          
%[13] "Cameroon"           "Chad"               "Chile"              "China"             
%[17] "Colombia"           "Congo, Dem. Rep."   "Congo, Rep."        "Costa Rica"        
%[21] "Cote d'Ivoire"      "Cuba"               "Dominican Republic" "Ecuador"           
%[25] "Egypt, Arab Rep."   "El Salvador"        "Ethiopia"           "Georgia"           
%[29] "Ghana"              "Guatemala"          "Guinea"             "Haiti"             
%[33] "Honduras"           "India"              "Indonesia"          "Iran, Islamic Rep."
%[37] "Iraq"               "Jordan"             "Kenya"              "Korea, Rep."       
%[41] "Lebanon"            "Liberia"            "Libya"              "Madagascar"        
%[45] "Malawi"             "Malaysia"           "Mali"               "Mauritania"        
%[49] "Mexico"             "Mongolia"           "Morocco"            "Mozambique"        
%[53] "Myanmar"            "Nepal"              "Nicaragua"          "Niger"             
%[57] "Nigeria"            "Pakistan"           "Panama"             "Paraguay"          
%[61] "Peru"               "Philippines"        "Portugal"           "Russian Federation"
%[65] "Rwanda"             "Saudi Arabia"       "Senegal"            "Serbia"            
%[69] "Sierra Leone"       "Singapore"          "South Africa"       "Sudan"             
%[73] "Tanzania"           "Thailand"           "Togo"               "Tunisia"           
%[77] "Turkey"             "Uganda"             "Ukraine"            "Uruguay"           
%[81] "Uzbekistan"         "Venezuela, RB"      "Vietnam"            "Yemen, Rep."       
%[85] "Zambia"             "Zimbabwe"           
%\end{verbatim}
%
%\noindent
%{\bf Countries where $Q_i^{\top}\hat \psi^s > 0$: }
%\begin{verbatim} 
%Groups where $Q_i^{\top}\hat \psi^s > 0$: 
%[1] "Algeria"              "Australia"            "Austria"             
% [4] "Belgium"              "Canada"               "Czech Republic"      
% [7] "Denmark"              "Finland"              "France"              
%[10] "Germany"              "Greece"               "Hungary"             
%[13] "Ireland"              "Israel"               "Italy"               
%[16] "Japan"                "Kazakhstan"           "Kuwait"              
%[19] "Netherlands"          "New Zealand"          "Norway"              
%[22] "Oman"                 "Poland"               "Romania"             
%[25] "Spain"                "Sweden"               "Switzerland"         
%[28] "United Arab Emirates" "United Kingdom"       "United States"       
%\end{verbatim}
%First we regress $Y$ on $X$ using those training examples for which $Q_i^{\top}\hat \psi^s \le 0$. We have the following result: 
%\begin{verbatim}
%Call:
%lm(formula = Y_poor ~ X_poor - 1)
%
%Residuals:
%    Min      1Q  Median      3Q     Max 
%-5.4250 -0.4588 -0.0581  0.4216  7.1246 
%
%Coefficients:
%                       Estimate Std. Error t value Pr(>|t|)    
%X_poorgdp_ave_vec       7.22097    0.79267   9.110 3.94e-14 ***
%X_poor                 -1.03085    0.15171  -6.795 1.53e-09 ***
%X_poorUrban_agglo_2015 -0.01954    0.01597  -1.223    0.225    
%---
%Signif. codes:  0 ‘***’ 0.001 ‘**’ 0.01 ‘*’ 0.05 ‘.’ 0.1 ‘ ’ 1
%
%Residual standard error: 1.972 on 83 degrees of freedom
%Multiple R-squared:  0.7692,	Adjusted R-squared:  0.7608 
%F-statistic: 92.18 on 3 and 83 DF,  p-value: < 2.2e-16
%\end{verbatim}
%
%\noindent
%And for the countries with $Q_i^{\top}\hat \psi^s > 0$: 
%\begin{verbatim}
%Call:
%lm(formula = Y_rich ~ X_rich - 1)
%
%Residuals:
%    Min      1Q  Median      3Q     Max 
%-7.7724 -1.9426 -0.3193  2.6936  9.0144 
%
%Coefficients:
%                       Estimate Std. Error t value Pr(>|t|)    
%X_richgdp_ave_vec       1.75096    0.90274   1.940  0.06294 .  
%X_rich                 -0.17986    0.12028  -1.495  0.14642    
%X_richUrban_agglo_2015  0.20404    0.05016   4.068  0.00037 ***
%---
%Signif. codes:  0 ‘***’ 0.001 ‘**’ 0.01 ‘*’ 0.05 ‘.’ 0.1 ‘ ’ 1
%
%Residual standard error: 4.169 on 27 degrees of freedom
%Multiple R-squared:  0.8641,	Adjusted R-squared:  0.849 
%F-statistic: 57.22 on 3 and 27 DF,  p-value: 7.926e-12
%\end{verbatim}
We illustrate our method using cross-country data on pollution (carbon-di-oxide), income and urbanization obtained from the World Development Indicators (WDI), World Bank (website?). The Environmental Kuznets Curve hypothesis (EKC henceforth), a popular and ongoing area of research in environmental economics, posits that at an initial stage of economic development pollution increases with economic growth, and then diminishes when society’s priorities change, leading to an inverted U-shaped relation between income (measured via real GDP per capita) and pollution. The hypothesis has led to numerous empirical papers (i) testing the hypothesis (whether the relation is inverted U-shaped for countries/regions of interest in the sample), (ii) exploring the threshold level of income (change point) at which pollution starts falling, as well as (iii) examining the countries/regions which belong to the upward rising part versus the downward sloping part of the inverted U-shape, if at all. The studies have been performed using US state level data or cross-country data (e.g. \cite{shafik1992economic}, \cite{millimet2003environmental}, \cite{aldy2005environmental}, \cite{lee2019nonparametric},\cite{boubellouta2021cross}, \cite{list1999environmental}, \cite{grossman1995economic}, \cite{bertinelli2005environmental}, \cite{azomahou2006economic}, \cite{taskin2000searching} to name a few) and most have found strong evidence in favor of the EKC hypothesis. While regressing pollution emission per capita on income and its squared term, most studies find a significantly positive effect of income and a significantly negative effect of its quadratic term on pollution, thus concluding in favor of the inverted U-shapedness of the relation.
\\\\
\noindent
While income-pollution remains the focal point of most EKC studies, several of them have also included urban agglomeration (UA) or some other measures of urbanization as an important control variable especially while investigating carbon emissions.\footnote{Although income growth is connected to urbanization, they are different due to varying geographical area, population density, and infrastructure of the countries. Also, different countries follow different income growth paths – labor intensive manufacturing, technology based manufacturing, human capital based servicing, technology based service sector, or natural resource (oil) based growth owing to their differences in terms of location, ownership of natural resources and capital.} (see for example, \cite{shafik1992economic}, \cite{boubellouta2021cross}, \cite{liang2019urbanization}). The ecological economics literature finds mixed evidence in this regard – (i) urbanization leading to more pollution (due to its close links with sanitation or dense transportations issues and proximities to polluting manufacturing industries), (ii) urbanization leading to less pollution (explained by ‘compact city theory’). The ‘compact city theory’ (see \cite{burton2000compact}, \cite{capello2000beyond}, \cite{sadorsky2014effect}) explains the benefits of increased urbanization in terms of economies of scale (for example, replacing dependence on automobiles with subway systems, the use of costlier but improved and green technology for basic infrastructure etc). \cite{cole2004examining}, using a set of 86 countries, and \cite{liddle2010age}, using 17 developed countries, find a positive and significant effect of urbanization on pollution. On the contrary, using a set of 69 countries \cite{sharma2011determinants} find a negative and significant effect of urbanization on pollution while \cite{du2012economic} find an insignificant effect of urbanization on carbon emission in China. Using various empirical strategies \cite{sadorsky2014effect} conclude that the positive and negative effects of urbanization on carbon pollution may cancel out depending on the countries involved, often leaving insignificant effects on pollution.  In summary, based on the existing literature, the relationship between urbanization and pollution relation appears to depend largely on the set of countries considered in the sample. This motivates us to use UA along with income in our change plane model for analyzing carbon-dioxide emission to plausibly separate the countries into two regimes. 
\\\\
\noindent
Following the broad literature we use pollution emission per capita (carbon-dioxide measured in metric tons per capita) as the dependent variable and real GDP per capita (measured in 2010 US dollars), its square (as is done commonly in the EKC literature) and a popular measure of urbanization, namely urban agglomeration  (UA)\footnote{The exact definition can be found in WDI website} as covariates (in our notation $X$) in our regression. In light of the preceding discussions we fit a change plane model comprising real GDP per capita and UA (in our notation $Q$). To summarize the setup, we use the continuous response model as described in equation \eqref{eq:regression_main_eqn}, i.e 
\begin{align*}
Y_i & = X_i^{\top}\beta_0 + X_i^{\top}\delta_0\mathds{1}_{Q_i^{\top}\psi_0 > 0} + \eps_i \\
& = X_i^{\top}\beta_0\mathds{1}_{Q_i^{\top}\psi_0 \le 0} + X_i^{\top}(\beta_0 + \delta_0)\mathds{1}_{Q_i^{\top}\psi_0 > 0} + \eps_i
\end{align*}
with the per capita $CO_2$ emission in metric ton as $Y$, per capita GDP, square of per capita GDP and UA as $X$ (hence $X \in \bbR^3$) and finally, per capita GDP and UA as $Q$ (hence $Q \in \bbR^2$). Observe that $\beta_0$ represents the regression coefficients corresponding to the countries with $Q_i^{\top}\psi_0 \le 0$ (henceforth denoted by Group 1) and $(\beta_0+ \delta_0)$ represents the regression coefficients corresponding to the countries with $Q_i^{\top}\psi_0 \ge 0$ (henceforth denoted by Group 2). As per our convention, in the interests of identifiability we assume $\psi_{0, 1} = 1$, where $\psi_{0,1}$ is the change plane parameter corresponding to per capita GDP. Therefore the only change plane coefficient to be estimated is $\psi_{0, 2}$, the change plane coefficient for UA. For numerical stability, we divide per capita GDP by $10^{-4}$ (consequently square of per capital GDP is scaled by $10^{-8}$)\footnote{This scaling helps in the numerical stability of the gradient descent algorithm used to optimize the least squares criterion.}.  After some pre-processing (i.e. removing rows consisting of NA and countries with $100\%$ UA) we estimate the coefficients $(\beta_0, \delta_0, \psi_0)$ of our model based on data from 115 countries with $\sigma_n = 0.05$ and test the significance of the various coefficients using the methodologies described in Section \ref{sec:inference}. We present our findings in Table \ref{tab:ekc_coeff}.  
\begin{table}[!h]
    \centering
    \begin{tabular}{|c||c||c|}
    \hline
    Coefficients & Estimated values & p-values \\
    \hline \hline 
      $\beta_{0, 1}$ (\text{RGDPPC for Group 1})  & 6.98555060 & 4.961452e-10   \\
       $\beta_{0, 2}$ (\text{squared RGDPPC for Group 1})  &  -0.43425991 & 7.136484e-02 \\
       $\beta_{0, 3}$ (\text{UA for Group 1}) & -0.02613813  & 1.066065e-01
\\
       $\beta_{0, 1} + \delta_{0, 1}$ (\text{RGDPPC for Group 2}) & 2.0563337 & 0.000000e+00\\
      $\beta_{0, 2} + \delta_{0, 2}$ (\text{squared RGDPPC for Group 2}) &  -0.1866490 & 4.912843e-04   \\
       $\beta_{0, 3} + \delta_{0, 3}$ (\text{UA for Group 2}) & 0.1403171& 1.329788e-05 \\
       $\psi_{0,2 }$  (\text{Change plane coeff for UA}) & -0.07061785 & 0.000000e+00\\
         \hline
    \end{tabular}
    \caption{Table of the estimated regression and change plane coefficients along with their p-values.}
    \label{tab:ekc_coeff}
\end{table}
%\begin{figure}
%\centering
%\includegraphics[scale=0.15]{Plots/World_map.png}
%\caption{A world map view of the countries in both the groups. Countries in Group 1 are indicated by green and countries in Group 2 are indicated by red. It is immediate that Group 2 mostly consists of developed countries (e.g. USA, UK, Germany etc.) and Group 1 primarily comprises emerging and under-developed countries like India, Angola etc.}
%\label{fig:world_map}
%\end{figure}
\\\\
\noindent
From the above analysis, we find that both GDP and its square have statistically significant effects on carbon pollution for both groups of countries with their expected signs (positive for GDP and negative for its square term), supporting the inverted U-shaped income-pollution nexus and being in line with most papers in the EKC literature.  The urban variable, on the other hand, is seen to have insignificant effect on Group 1 countries  (less developed and emerging) which is in keeping with \cite{du2012economic}, \cite{sadorsky2014effect}. However, the urban variable seems to have a positive and significant impact on Group-2 countries which is in line with \cite{liddle2010age} for example. Note that many of the group-1 countries are yet to experience sizeable levels of urbanization compared to the other group and this is even truer for our sample period.\footnote{We use 6 years average from 2010-2015 for GDP and pollution measures. Such averaging is in accordance with the cross-sectional empirical literature using cross-country/regional data and helps avoid business cycle fluctuations in GDP. It also minimizes the impacts of outlier events such as the financial crisis or great recession period.  The years that have we have chosen are ones for which we could find data for the largest number of countries.}Further, note that UA plays a crucial role in dividing the countries into different regimes, as the estimated value of $\psi_{0,2}$ is significant.   
\\\\
\noindent
There are many future potential applications of our method in economics. Similar exercises can be followed for other pollutants (such as sulfur emission, electrical waste/e-waste, nitrogen pollution etc.). While income/GDP remains a common, indeed the most crucial variable in the pollution study, other covariates (including change plane defining variables) may vary, depending on the pollutant of interest. One may also be interested in the determinants of health expenses in the household survey data. Often the families are asked about their health expenses incurred in the past one year. An interesting case in point may be household surveys collected in India where there are many large joint families with several children and old people live in the same household and most families are uninsured. It is often seen that health expenses increases with income as it includes expenses on regularly performed preventative medical examinations which are affordable only beyond an income level is reached. The important covariates are per capita family income, family wealth, 'dependency ratio' (number of children and old to the total number of people in the family) and binary indicator of any history of major illness/hospitalizations in the family in the past year. Family income per capita and history of major illness can potentially define the change plane.
%One may also be interested in the determinants of medical migration in the context of medical brain-drain literature. Determinants of bilateral emigration of physicians and other health personnel from a set of developing countries to several developed countries are studied in the literature. Apart from important covariates like GDP differences, work-load differences, other interesting variables such as a binary indicator for common language spoken between the sender and the recipient countries as well as the degree of ‘networking’ (at both cultural and professional spheres indicated by the volume of existing immigrants from the sender to the recipient country) can help forming the change plane.  
\end{comment}


\input{Real_data_analysis.tex}
\section{Conclusion}
\label{sec:conclusion}
In this paper we have established that under some mild assumptions the kernel-smoothed change plane estimator is asymptotically normal with near optimal rate $n^{-1}$. To the best of our knowledge, the state of the art result in this genre of problems is due to \cite{seo2007smoothed}, where they demonstrate a best possible rate about $n^{-3/4}$ for i.i.d. data. The main difference between their approach and ours is mainly the proof of Lemma \ref{bandwidth}. Our techniques are based upon modern empirical process theory which allow us to consider much smaller bandwidths $\sigma_n$ compared to those in \cite{seo2007smoothed}, who appear to require larger values to achieve the result, possibly owing to their reliance on the techniques developed in \cite{horowitz1992smoothed}. Although we have established it is possible to have asymptotic normality with really small bandwidths, we believe that the finite sample approximation (e.g. Berry-Essen bound) to normality could be poor, which is also evident from our simulation. 
%Therefore in practice it is preferable to use larger bandwidth if inference is the main 


%\appendix




==> Upload materials/regression.tex <==
% !TEX root = Final_draft.tex
\renewcommand{\th}{\theta}
\section{Methodology and Theory for Continuous Response Model}
\label{sec:theory_regression}
In this section we present our analysis for the continuous response model. Without smoothing, the original estimating equation is: 
$$
f_{\beta, \delta, \psi}(Y, X, Q) = \left(Y - X^{\top}\beta - X^{\top}\delta\mathds{1}_{Q^{\top}\psi > 0}\right)^2  
$$
and we estimate the parameters as: 
\begin{align}
\label{eq:ls_estimator}
\left(\hat \beta^{LS}, \hat \delta^{LS}, \hat \psi^{LS}\right) & = \argmin_{(\beta, \delta, \psi) \in \Theta} \bbP_n f_{\beta, \delta, \psi} \notag \\
& :=  \argmin_{(\beta, \delta, \psi) \in \Theta}\bbM_n(\beta, \delta, \psi)\,.
\end{align}
where $\bbP_n$ is empirical measure based on i.i.d. observations $\{(X_i, Y_i, Q_i)\}_{i=1}^n$ and $\Theta$ is the parameter space. Henceforth, we assume $\Theta$ is a compact subset of dimension $\reals^{2p+d}$. We also define $\theta = (\beta, \delta, \psi)$, i.e. all the parameters together as a vector and by $\theta_0$ is used to denote the true parameter vector $(\beta_0, \delta_0, \psi_0)$. Some modification of equation \eqref{eq:ls_estimator} leads to the following:  
\begin{align*}
(\hat \beta^{LS}, \hat \delta^{LS}, \hat \psi^{LS}) & = \argmin_{\beta, \delta, \psi}  \sum_{i=1}^n \left(Y_i - X_i^{\top}\beta - X_i^{\top}\delta\mathds{1}_{Q_i^{\top}\psi > 0}\right)^2 \\ 
& = \argmin_{\beta, \delta, \psi}  \sum_{i=1}^n \left[\left(Y_i - X_i^{\top}\beta\right)^2\mathds{1}_{Q_i^{\top}\psi_0 \le 0} \right. \\
&  \hspace{14em} \left. + \left(Y_i - X_i^{\top}\beta - X_i^{\top}\delta\right)^2\mathds{1}_{Q_i^{\top}\psi > 0} \right] \\
& = \argmin_{\beta, \delta, \psi}  \sum_{i=1}^n \left[\left(Y_i - X_i^{\top}\beta\right)^2 + \left\{\left(Y_i - X_i^{\top}\beta - X_i^{\top}\delta\right)^2 \right. \right. \\
& \hspace{17em} \left. \left. - \left(Y_i - X_i^{\top}\beta\right)^2\right\}\mathds{1}_{Q_i^{\top}\psi > 0} \right] 
\end{align*}
Typical empirical process calculations yield under mild conditions: 
$$
\|\hat \beta^{LS} - \beta_0\|^2 + \|\hat \delta^{LS} - \delta_0\|^2 + \|\hat \psi^{LS} - \psi_0 \|_2 = O_p(n^{-1})
$$
but inference is difficult as the limit distribution is unknown, and in any case, would be a highly non-standard distribution. Recall that even in the one-dimensional change point model with fixed jump size, the least squares change point estimator converges at rate $n$ to the truth with a non-standard limit distribution, namely a minimizer of a two-sided compound Poisson process (see \cite{lan2009change} for more details). To obtain a computable estimator with tractable limiting distribution, we resort to a smooth approximation of the indicator function in \eqref{eq:ls_estimator} using a distribution kernel with suitable bandwidth, i.e we replace $\mathds{1}_{Q_i^{\top}\psi > 0}$ by $K(Q_i^{\top}\psi/\sigma_n)$ for some appropriate distribution function $K$ and bandwidth $\sigma_n$, i.e. 
\begin{align*}
(\hat \beta^S, \hat \delta^S, \hat \psi^S) & = \argmin_{\beta, \delta, \psi} \left\{ \frac1n \sum_{i=1}^n \left[\left(Y_i - X_i^{\top}\beta\right)^2 + \left\{\left(Y_i - X_i^{\top}\beta - X_i^{\top}\delta\right)^2 \right. \right. \right. \\
& \hspace{15em} \left. \left. \left. - \left(Y_i - X_i^{\top}\beta\right)^2\right\}K\left(\frac{Q_i^{\top}\psi}{\sigma_n}\right) \right] \right\} \\
& = \argmin_{(\beta, \delta, \psi) \in \Theta} \bbP_n f^s_{(\beta, \delta, \psi)}(X, Y, Q) \\
& := \argmin_{\theta \in \Theta} \bbM^s_n(\theta) \,.
\end{align*}
%We minimize the following squared error loss function to estimate the parameters: 
%\begin{align*}
%(\hat \beta, \hat \delta, \hat \psi) & = \argmin_{\beta, \delta, \psi} \frac1n \sum_i \left(Y_i - X_i^{\top}\beta -  X_i^{\top}\delta\mathds{1}_{Q_i^{\top}\psi > 0} \right)^2 \\
%& =\argmin_{\beta, \delta, \psi}  \frac{1}{n}\sum_{i=1}^n \left(Y_i - X_i^{\top}\beta\right)^2 \mathds{1}_{Q_i^{\top}\psi \le 0} + \frac{1}{n}\sum_{i=1}^n \left(Y_i - X_i^{\top}(\beta + \delta)\right)^2 \mathds{1}_{Q_i^{\top}\psi > 0}  \\
%    & = \argmin_{\beta, \delta, \psi}  \frac{1}{n}\sum_{i=1}^n \left(Y_i - X_i^{\top}\beta\right)^2 + \frac{1}{n}\sum_{i=1}^n \left[\left(Y_i - X_i^{\top}(\beta + \delta)\right)^2 - \left(Y_i - X_i^{\top}\beta\right)^2  \right] \mathds{1}_{Q_i^{\top}\psi > 0} \\
%    \label{eq:non_smooth} & = \argmin_{\beta, \delta, \psi}  \frac{1}{n}\sum_{i=1}^n \left(Y_i - X_i^{\top}\beta\right)^2 + \frac{1}{n}\sum_{i=1}^n \left[-2\left(Y_i - X_i^{\top}\beta\right)X_i^{\top}\delta + (X_i^{\top}\delta)^2\right] \mathds{1}_{Q_i^{\top}\psi > 0} \\
%& := \argmin_{\beta, \delta, \psi} \ \ \bbM_n(\th) \,. 
%\end{align*}
%where by $\th$ we denote the vector of all parameters $(\beta, \delta, \psi)$. However due to presence of an indicator function the above optimization problem is NP-hard and the asymptotic distribution of the estimator is (almost) intractable for all practical purposes. One way to circumvent this issue is to replace the indicator function by a smooth kernel and then apply gradient descent to optimize the parameters. The empirical smoothed loss function is defined as: 
%%$$
%%\bbM_n^s(\theta) = \bbE\left[(Y - X^{\top}\beta)^2 + \left\{-2(Y-X^{\top}\beta)(X^{\top}\delta) + (X^{\top}\delta)^2\right\}K\left(\frac{Q^{\top}\psi}{\sigma_n}\right)\right] \,.
%%$$
%\begin{align}
%\bbM_n^s(\theta) & = \left\{ \frac{1}{n}\sum_{i=1}^n \left(Y_i - X_i^{\top}\beta\right)^2 + \frac{1}{n}\sum_{i=1}^n \left[-2\left(Y_i - X_i^{\top}\beta\right)X_i^{\top}\delta \right. \right. \notag \\
%& \hspace{20em} \left. \left. + (X_i^{\top}\delta)^2\right] K\left(\frac{Q^{\top}\psi}{\sigma_n}\right)\right\}\,.
%\end{align}
%and the corresponding smoothed estimator as: 
%$$
%(\hat \beta^s, \hat \delta^s, \hat \psi^s) = \argmin_{\beta, \delta, \psi} \bbM_n^s(\theta) \,.
%$$
%
%
%\begin{align}
%    \hat \theta_n^s := (\hat \beta^s, \hat \delta^s, \hat \psi^s) & = \argmin_{\beta, \delta, \psi} \frac1n \sum_i \left(Y_i - X_i^{\top}\beta - X_i^{\top}\delta K\left(\frac{Q_i^{\top}\psi}{\sigma_n}\right) \right)^2 \\
%     & =\argmin_{\beta, \delta, \psi}  \frac{1}{n}\sum_{i=1}^n \left(Y_i - X_i^{\top}\beta\right)^2 \mathds{1}_{Q_i^{\top}\psi \le 0} + \frac{1}{n}\sum_{i=1}^n \left(Y_i - X_i^{\top}(\beta + \delta)\right)^2 \mathds{1}_{Q_i^{\top}\psi > 0}  \\
%    & = \argmin_{\beta, \delta, \psi}  \frac{1}{n}\sum_{i=1}^n \left(Y_i - X_i^{\top}\beta\right)^2 + \frac{1}{n}\sum_{i=1}^n \left[\left(Y_i - X_i^{\top}(\beta + \delta)\right)^2 - \left(Y_i - X_i^{\top}\beta\right)^2  \right] \mathds{1}_{Q_i^{\top}\psi > 0} \\
%    \label{eq:non_smooth} & = \argmin_{\beta, \delta, \psi}  \frac{1}{n}\sum_{i=1}^n \left(Y_i - X_i^{\top}\beta\right)^2 + \frac{1}{n}\sum_{i=1}^n \left[-2\left(Y_i - X_i^{\top}\beta\right)X_i^{\top}\delta + (X_i^{\top}\delta)^2\right] \mathds{1}_{Q_i^{\top}\psi > 0} \\
%    & := \argmin_{\beta, \delta, \psi} \ \ \bbM^s_n(\beta, \delta, \psi) \,. 
%\end{align}
Define $\bbM$ (resp. $\bbM^s$) to be the population counterpart of $\bbM_n$ and $\bbM_n^s$ respectively which are defined as: 
\begin{align*}
\bbM(\th) & = \bbE\left(Y - X^{\top}\beta\right)^2 + \bbE\left(\left[-2\left(Y_i - X^{\top}\beta\right)X^{\top}\delta + (X^{\top}\delta)^2\right] \mathds{1}_{Q^{\top}\psi > 0}\right) \,, \\
\bbM^s(\theta) & = \bbE\left[(Y - X^{\top}\beta)^2 + \left\{-2(Y-X^{\top}\beta)(X^{\top}\delta) + (X^{\top}\delta)^2\right\}K\left(\frac{Q^{\top}\psi}{\sigma_n}\right)\right] \,.
\end{align*}
%We approach the estimation problem from empirical process point of view and try to prove the following theorem:
%\begin{theorem}
%\label{thm:regression}
%Under a proper choice of kernel and certain assumptions on the distribution of $(X, Q, \eps)$: 
%$$
%\begin{pmatrix}
%\sqrt{n}\left(\hat \beta^s - \beta_0\right) \\
%\sqrt{n}\left(\hat \delta^s - \delta_0\right) \\
%\sqrt{n/\sigma_n} \left(\hat \psi^s - \psi_0\right) 
%\end{pmatrix} \overset{\mathscr{L}}{\implies} \cN(0, \Sigma) \,.
%$$
%as long as $n \sigma_n \to \infty$. 
%\end{theorem}
As noted in the proof of \textcolor{blue}{Seo and Linton}, the assumption $\log{n}/n\sigma_n^2 \to 0$ was only used to show: 
$$
\frac{\left\|\hat \psi^s - \psi_0\right\|}{\sigma_n} = o_p(1) \,.
$$
In this paper, we show that one can achieve the same conclusion as long as $n\sigma_n \to \infty$.  The rest of the proof for the normality is similar to that of \cite{seo2007smoothed}, we will present it briefly for the ease the readers. The proof is quite long and technical, therefore we break the proof into several lemmas. We, first, list our assumptions: 
\begin{assumption}
\label{eq:assm}
%We need the following assumptions on the distribution of $(X, Q)$: 
\begin{enumerate}
\item Define $f_\psi(\cdot \mid \tilde Q)$ to be the conditional distribution of $Q^{\top}\psi$ given $\tilde Q$. (In particular we will denote by $f_0(\cdot \mid \tilde q)$ to be conditional distribution of $Q^{\top}\psi_0$ given $\tilde Q$ and $f_s(\cdot \mid \tilde q)$ to be the conditional distribution of $Q^{\top}\psi_0^s$ given $\tilde Q$. Assume that there exists $F_+$ such that $\sup_t f_0(t | \tilde Q) \le F_+$ almost surely on $\tilde Q$ and for all $\psi$ in a neighborhood of $\psi_0$ (in particular for $\psi_0^s$). Further assume that $f_\psi$ is differentiable and the derivative is bounded by $F_+$ for all $\psi$ in a neighborhood of $\psi_0$ (again in particular for $\psi_0^s$).
\vspace{0.1in}
\item Define $g(Q) = \var(X \mid Q)$. There exists $c_-$ and $c_+$ such that $c_- \le \lambda_{\min}(g(Q)) \le \lambda_{\max}(g(Q)) \le c_+$ almost surely. Also assume that $g$ is a Lipschitz with constant $G_+$ with respect to $Q$. 
\vspace{0.1in}
\item There exists $p_+ < \infty$ and $p_- > 0, r > 0$ such that: 
$$
p_- \|\psi - \psi_0\| \le \bbP\left(\s\left(Q^{\top}\psi\right) \neq \s\left(Q^{\top}\psi_0\right)\right) \le p_+ \|\psi - \psi_0\| \,,
$$
for all $\psi$ such that $\|\psi - \psi_0\| \le r$. 
\vspace{0.1in}
\item For all $\psi$ in the parameter space $0 < \bbP\left(Q^{\top}\psi > 0\right) < 1$. 
\vspace{0.1in} 
\item Define $m_2(Q) = \bbE\left[\|X\|^2 \mid Q\right]$ and $m_4(Q) = \bbE\left[\|X\|^4 \mid Q\right]$. Assume $m_2, m_4$ are bounded Lipschitz function of $Q$.  
\end{enumerate}
\end{assumption}


\subsection{Sufficient conditions for above assumptions }
We now demonstrate some sufficient conditions for the above assumptions to hold. The first condition is essentially a condition on the conditional density of the first co-ordinate of $Q$ given all other co-ordinates. If this conditional density is bounded and has bounded derivative, then first assumption is satisfied. This condition is satisfied in fair generality. The second assumption implies that the conditional distribution of X given Q has variance in all the direction over all $Q$. This is also very weak condition, as is satisfied for example if X and Q and independent (with $X$ has non-degenerate covariance matrix) or $(X, Q)$ are jointly normally distributed to name a few. This condition can further be weaken by assuming that the maximum and minimum eigenvalues of $\bbE[g(Q)]$ are bounded away from $\infty$ and $0$ respectively but it requires more tedious book-keeping. The third assumption is satisfied as long as as $Q^{\top}\psi$ has non-zero density near origin, while the fourth assumption merely states that the support of  $Q$ is not confined to one side of the hyperplane for any hyperplane and a simple sufficient condition for this is $Q$ has continuous density with non-zero value at the origin. The last assumption is analogous to the second assumption for the conditional fourth moment which is also satisfied in fair generality. 
%If the support of $X$ is compact and both $f_1(\cdot | \tilde X)$ and $f'_1(\cdot | \tilde X)$ are uniformly bounded in $\tilde X$, then Assumptions $(\ref{as:distribution}, \ \ref{as:differentiability}, \ \ref{as:density_bound},\ \ref{as:derivative_bound})$ follow immediately. The first part of Assumption \ref{as:eigenval_bound}, i.e. the assumption $f_{\tilde{Q}}(0) > 0$ is also fairly general and satisfied by many standard probability distributions. The second part of Assumption \ref{as:eigenval_bound} is satisfied when $f_0(0|\tilde{Q})$ has some lower bound independent of $\tilde{Q}$ and $\tilde{Q}$ has non-singular dispersion matrix. Assumption \ref{as:kernel} is a standard assumption on the kernel and is satisfied for a large class of distribution functions, e.g. $k(x) = (3/4)(1-x^2)$ on $[-1.1]$. 
\\\\
\noindent
{\bf Kernel function and bandwidth: } We take $K(x) = \Phi(x)$ (distribution of standard normal random variable) for our analysis. For the bandwidth we assume $n\sigma_n^2 \to 0$ and $n \sigma_n \to \infty$ as the other case, (i.e. $n\sigma_n^2 \to \infty$) is already established in \cite{seo2007smoothed}. 
\\\\
\noindent
Based on Assumption \ref{eq:assm} and our choice of kernel and bandwidth we establish the following theorem: 
\begin{theorem}
\label{thm:regression}
Under Assumption \ref{eq:assm} and the above choice of kernel and bandwidth we have: 
%$$
%\begin{pmatrix}
%\sqrt{n}\left(\hat \beta^s - \beta_0\right) \\
%\sqrt{n}\left(\hat \delta^s - \delta_0\right) \\
%\sqrt{n/\sigma_n} \left(\hat \psi^s - \psi_0\right) 
%\end{pmatrix} \overset{\mathscr{L}}{\implies} \cN(0, \Sigma) \,.
%$$
$$
\sqrt{n}\begin{pmatrix}\begin{pmatrix} \hat \beta^s \\ \hat \delta^s \end{pmatrix} - \begin{pmatrix} \beta_0 \\ \delta_0 \end{pmatrix} \end{pmatrix} \overset{\mathscr{L}}{\implies} \cN(0, \Sigma_{\beta, \delta})
$$
and 
$$
\sqrt{n/\sigma_n} \left(\hat \psi^s - \psi_0\right) \overset{\mathscr{L}}{\implies} \cN(0, \Sigma_\psi) \,,
$$
for matrices $\Sigma_{\beta, \delta}$ and $\Sigma_\psi$ mentioned explicitly in the proof. Moreover they are asymptotically independent. 
\end{theorem}
The proof of the theorem is relatively long, so we break it into several lemmas. We  provide a roadmap of the proof in this section while the elaborate technical derivations of the supporting lemmas can be found in Appendix. Let $\nabla \bbM_n^s(\theta)$ and $\nabla^2 \bbM_n^s(\theta)$ be the gradient and Hessian of $\bbM_n^s(\theta)$ with respect to $\theta$.  As $\hat \theta^s$ minimizes $\bbM_n^s(\theta)$, we have from the first order condition, $\nabla \bbM_n^s(\hat \theta^s) = 0$. Using one step Taylor expansion we have:
\allowdisplaybreaks 
\begin{align*}
\label{eq:taylor_first}
\nabla \bbM_n^s(\hat \theta^s) = \nabla \bbM_n^s(\theta_0) + \nabla^2 \bbM_n^s(\theta^*)\left(\hat \theta^s - \theta_0\right) = 0
\end{align*}
i.e.
\begin{equation}
\label{eq:main_eq}  
\left(\hat{\theta}^s - \theta_0\right) = -\left(\nabla^2 \bbM_n^s(\theta^*)\right)^{-1} \nabla \bbM_n^s(\theta_0)
\end{equation}
for some intermediate point $\th^*$ between $\hat \theta^s$ and $\theta_0$. 
Following the notation of \cite{seo2007smoothed}, define a diagonal matrix $D_n$ of dimension $2p + d$ with first $2p$ elements being 1 and the last $d$ elements being $\sqrt{\sigma_n}$. 
 we can write: 
\begin{align}
\sqrt{n}D_n^{-1}(\hat \theta^s - \theta_0) & = - \sqrt{n}D_n^{-1}\nabla^2\bbM_n^s(\theta^*)^{-1}\nabla \bbM_n^s(\theta_0)  \notag \\
\label{eq:taylor_main} & = \begin{pmatrix} \nabla^2\bbM_n^{s, \gamma}(\theta^*) & \sqrt{\sigma_n}\nabla^2\bbM_n^{s, \gamma \psi}(\theta^*) \\
\sqrt{\sigma_n}\nabla^2\bbM_n^{s, \gamma \psi}(\theta^*) & \sigma_n\nabla^2\bbM_n^{s, \psi}(\theta^*)\end{pmatrix}^{-1}\begin{pmatrix} \sqrt{n}\nabla \bbM_n^{s, \gamma}(\theta_0) \\ \sqrt{n\sigma_n}\nabla \bbM_n^{s, \psi}(\theta_0)\end{pmatrix}
\end{align}
where $\gamma = (\beta, \delta) \in \reals^{2p}$. The following lemma establishes the asymptotic properties of $\nabla \bbM_n^s(\theta_0)$: 
\begin{lemma}[Asymptotic Normality of $\nabla \bbM_n^s(\theta_0)$]
\label{asymp-normality}
%\begin{lemma}
\label{asymp-normality}
Under assumption \ref{eq:assm} we have: 
%$$
%\sqrt{n \sigma_n} T_n(\theta_0) \Rightarrow \mathcal{N}(\mu, \Sigma)
%$$
\begin{align*}
\sqrt{n}\nabla \bbM_n^{s, \gamma}(\theta_0) \implies \cN\left(0, 4V^{\gamma}\right) \,,\\
\sqrt{n\sigma_n}\nabla \bbM_n^{s, \psi}(\theta_0) \implies \cN\left(0, V^{\psi}\right) \,.
\end{align*} 
for some n.n.d. matrices $V^{\gamma}$ and $V^{\psi}$ which is mentioned explicitly in the proof. Further more $\sqrt{n}\nabla \bbM_n^{s, \gamma}(\theta_0)$ and $\sqrt{n\sigma_n}\nabla \bbM_n^{s, \psi}(\theta_0)$ are asymptotically independent. 
\end{lemma}
\noindent
%If we take $\sigma_n$ to be close to $1/n$ say $\sigma_n = (\log{n})^2/n$ then $\lambda = 0$. 
%In the case that $n \sigma_n^3 \rightarrow 0$, which, holds when $\log n/(n\sigma_n) \rightarrow 0$ as assumed prior to the statement of the theorem, $\lambda = 0$ and we have: 
%$$\sqrt{n \sigma_n} T_n(\theta_0) \rightarrow \mathcal{N}(0, \Sigma) \,.$$ 
Next, we analyze the convergence of $\nabla^2 \bbM_n^s(\theta^*)$ which is stated in the following lemma: 
\begin{lemma}[Convergence in Probability of $\nabla^s \bbM_n^s(\th^*)$]
\label{conv-prob}
Under Assumption \eqref{eq:assm}, for any random sequence $\breve{\theta} = \left(\breve{\beta}, \breve{\delta}, \breve{\psi}\right)$ such that $\breve{\beta} \overset{p}{\to} \beta_0, \breve{\delta} \overset{p}{\to} \delta_0, \|\breve{\psi} - \psi_0\|/\sigma_n \overset{P} \rightarrow 0$, we have: 
\begin{align*}
\nabla^2_{\gamma} \bbM_n^s(\breve{\theta}) & \overset{p}{\longrightarrow} 2Q^{\gamma} \,, \\
\sqrt{\sigma_n}\nabla^2_{\psi \gamma} \bbM_n^s(\breve{\theta}) & \overset{p}{\longrightarrow} 0 \,, \\
\sigma_n \nabla^2_{\psi} \bbM_n^s(\breve{\theta}) & \overset{p}{\longrightarrow} Q^{\psi} \,.
\end{align*}
for some matrices $Q^{\gamma}, Q^{\psi}$ mentioned explicitly in the proof. This, along with equation \eqref{eq:taylor_main}, establishes: 
\begin{align*}
\sqrt{n}\left(\hat \gamma^s - \gamma_0\right) & \overset{\mathscr{L}}{\implies} \cN\left(0, Q^{\gamma^{-1}}V^{\gamma}Q^{\gamma^{-1}}\right) \,, \\
\sqrt{n/\sigma_n}\left(\hat \psi^s - \psi_0\right) & \overset{\mathscr{L}}{\implies} \cN\left(0, Q^{\psi^{-1}}V^{\psi}Q^{\psi^{-1}}\right) \,.
\end{align*}
where as before $\hat \gamma^s = (\hat \beta^s, \hat \delta^s)$. 
\end{lemma}
It will be shown later that the condition $\|\breve{\psi}_n - \psi_0\|/\sigma_n \overset{P} \rightarrow 0$ needed in Lemma \ref{conv-prob} holds for the (random) sequence $\psi^*$, the intermediate point in the Taylor expansion. Then, combining Lemma \ref{asymp-normality} and Lemma \ref{conv-prob} we conclude the proof of Theorem \ref{thm:regression}. %from equation \ref{eq:main_eq} that: $$\sqrt{n/\sigma_n} \left(\hat{\theta}_n - \theta_0\right) \Rightarrow N(0, Q^{-1}\Sigma Q^{-1})$$ This concludes the proof of the our Theorem \ref{main} with $\Gamma = Q^{-1}\Sigma Q^{-1}$. 
%\newline
%\newline
Observe that, to show $\left\|\psi^* - \psi_0 \right\| = o_P(\sigma_n)$, it suffices to to prove that $\left\|\hat \psi^s - \psi_0 \right\| = o_P(\sigma_n)$. Towards that direction, we have following lemma: 

\begin{lemma}[Rate of convergence]
\label{lem:rate_smooth}
Under Assumption \ref{eq:assm} and our choice of kernel and bandwidth, 
$$
n^{2/3}\sigma_n^{-1/3} d^2_*\left(\hat \theta^s, \theta_0^s\right) = O_P(1) \,,
$$
where 
\begin{align*}
d_*^2(\th, \th_0^s) & =  \|\beta - \beta_0^s\|^2 + \|\delta - \delta_0^s\|^2 \\
& \qquad \qquad + \frac{\|\psi - \psi_0^s\|^2}{\sigma_n} \mathds{1}_{\|\psi - \psi_0^s\| \le \cK\sigma_n} + \|\psi - \psi_0^s\| \mathds{1}_{\|\psi - \psi_0^s\| > \cK\sigma_n}  \,.
\end{align*}
for some specific constant $\cK$. (This constant will be mentioned precisely in the proof). Hence as $n\sigma_n \to \infty$, we have $n^{2/3}\sigma_n^{-1/3} \gg \sigma_n^{-1}$ which implies $\|\hat \psi^s - \psi_0^s\|/\sigma_n  \overset{P}  \longrightarrow 0 \,.$
\end{lemma}
%
%\noindent
%The lemma immediately leads to the following corollary: 
%
%\begin{corollary}
%\label{rate-cor}
%If $(\log{n})/(n\sigma_n)\rightarrow 0$ then $\frac{\|\hat{\theta}_n - \theta_n\|}{\sigma_n}  \overset{P}  \longrightarrow 0$
%\end{corollary}
%
\noindent
The above lemma establishes $\|\hat \psi^s - \psi_0^s\|/\sigma_n = o_p(1)$ but our goal is to show that $\|\hat \psi^s - \psi_0\|/\sigma_n = o_p(1)$. Therefore, we further need $\|\psi^s_0 - \psi_0\|/\sigma_n \rightarrow 0$ which is demonstrated in the following lemma:

\begin{lemma}[Convergence of population minimizer]
\label{bandwidth}
Under Assumption \ref{eq:assm} and our choice of kernel and bandwidth, we have: $\|\psi^s_0 - \psi_0\|/\sigma_n \rightarrow 0$. 
\end{lemma}

\noindent
Hence the final roadmap is the following: Using Lemma \ref{bandwidth} and Lemma \ref{lem:rate_smooth} we establish that $\|\hat \psi^s - \psi_0\|/\sigma_n = o_p(1)$ if $n\sigma_n \to 0$. This, in turn, enables us to prove Lemma \ref{conv-prob}, i.e. $\sigma_n \nabla^2 \bbM_n^s(\theta^*) \overset{P} \rightarrow Q$,which, along with Lemma \ref{asymp-normality}, establishes the main theorem. 







%Now we go back to our smoothed version of the change plane model. Note that the population version changes with $n$ as the bandwidth changes with $n$. The population loss function for the smoothed change point is: 
%$$
%\bbM^s(\theta) = \bbE\left[(Y - X^{\top}\beta)^2 + \left\{-2(Y-X^{\top}\beta)(X^{\top}\delta) + (X^{\top}\delta)^2\right\}K\left(\frac{Q^{\top}\psi}{\sigma_n}\right)\right] \,.
%$$
%where we simply replace the indicator of equation \eqref{eq:non_normal} by a distribution kernel. 
%













%\begin{lemma}
%\label{lem:rate_smooth}
%Under Assumption \ref{eq:assm} we have: 
%$$
%n^{2/3}\sigma_n^{-1/3}d^2_*(\hat \th^s, \th_0^s) = O_p(1) \,.
%$$
%where $d_*$ is the (semi)-metric defined in Lemma \ref{lem:pop_smooth_curvarture}. As a consequence, if $n\sigma_n \to \infty$, then $d^2_*(\hat \th^s, \th_0^s)/\sigma_n = o_p(1)$. 
%\end{lemma}
%
%
%
%\begin{lemma}
%\DM{Complete the proof of asymptotic normality}. 
%\end{lemma}

==> Upload materials/ykMacros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\be{\mathbf{e}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{{\sf subject\ to}}
\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> Upload materials/ykThmMacros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> ykMacros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\be{\mathbf{e}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{{\sf subject\ to}}
\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> ykThmMacros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}

